Data Driven Optimization of Inter-Frequency Mobility Parameters for Emerging Multi-band Networks

Densification and multi-band operation in 5G and beyond pose an unprecedented challenge for mobility management, particularly for inter-frequency handovers. The challenge is aggravated by the fact that the impact of key inter-frequency mobility parameters, namely A5 time to trigger (TTT), A5 threshold1 and A5 threshold2 on the system's performance is not fully understood. These parameters are fixed to a gold standard value or adjusted through hit and trial. This paper presents a first study to analyze and optimize A5 parameters for jointly maximizing two key performance indicators (KPIs): Reference signal received power (RSRP) and handover success rate (HOSR). As analytical modeling cannot capture the system-level complexity, a data driven approach is used. By developing XGBoost based model, that outperforms other models in terms of accuracy, we first analyze the concurrent impact of the three parameters on the two KPIs. The results reveal three key insights: 1) there exist optimal parameter values for each KPI; 2) these optimal values do not necessarily belong to the current gold standard; 3) the optimal parameter values for the two KPIs do not overlap. We then leverage the Sobol variance-based sensitivity analysis to draw some insights which can be used to avoid the parametric conflict while jointly maximizing both KPIs. We formulate the joint RSRP and HOSR optimization problem, show that it is non-convex and solve it using the genetic algorithm (GA). Comparison with the brute force-based results show that the proposed data driven GA-aided solution is 48x faster with negligible loss in optimality.

==> Tables.tex <==
\begin{table}[t]
\centering
\caption{Prediction of Mean RSRP}
\label{table:RSRPpred}
\begin{tabular}{|>{\centering\arraybackslash} m{2cm} | >{\centering\arraybackslash} m{1.5cm}| >{\centering\arraybackslash} m{1cm}| >{\centering\arraybackslash} m{1.5cm}|}
\hline
\textbf{Model} & \textbf{Root Mean Square Error (dBm)} & \textbf{R2 Score} & \textbf{Mean Cross-Validation Score}                \\ \hline
Linear Regression & 0.4613 & 0.6628 & 0.6798                    \\ \hline
Polynomial Regression & 0.1859 & 0.9452 & 0.6798                     \\ \hline
Support Vector Regression & 0.1228 & 0.9761 & 0.9784                    \\ \hline
Decision Tree Regression & 0.0930 & 0.9863 & 0.9859                     \\ \hline
Random Forest Regression & 0.0748 & 0.9911 & 0.9908                     \\ \hline
XGBoost Regression & 0.0737 & 0.9914 & 0.9919                 \\ \hline
\end{tabular}
\end{table}

\subsubsection{RLF Rate}
\begin{table}[t]
\centering
\caption{Prediction of Handover Success Rate}
\label{table:RLFpred}
\begin{tabular}{|>{\centering\arraybackslash} m{2cm} | >{\centering\arraybackslash} m{1.5cm}| >{\centering\arraybackslash} m{1cm}| >{\centering\arraybackslash} m{1.5cm}|}
\hline
\textbf{Model} & \textbf{Root Mean Square Error} & \textbf{R2 Score} & \textbf{Mean Cross-Validation Score}                \\ \hline
Linear Regression & 0.0559 & 0.4471 & 0.4556                    \\ \hline
Polynomial Regression & 0.0474 & 0.6026 & 0.4556                     \\ \hline
Support Vector Regression & 0.0495 & 0.5671 & 0.5610                    \\ \hline
Decision Tree Regression & 0.0337 & 0.7995 & 0.7177                     \\ \hline
Random Forest Regression & 0.0258 & 0.8826 & 0.8223                     \\ \hline
XGBoost Regression & 0.0250 & 0.8893 & 0.8304                 \\ \hline
\end{tabular}
\end{table}
